Scaling Parallel Sequence Models to Foundation-Scale Vision Encoders

Vision foundation models are bottlenecked by the quadratic cost of self-attention, which limits usable resolution and increases the cost of large-scale pretraining. Subquadratic alternatives such as linear attention and state-space models reduce this cost, but often serialize images into 1D token streams and weaken the 2D spatial structure important for vision. Generalized Spatial Propagation Networks (GSPN) instead propagate context directly on the 2D grid through line-scan recurrences, achieving near-linear complexity without positional embeddings, but have seen little use as foundation-scale encoders. We present C-GSPN, a foundation-scale vision encoder based on 2D spatial propagation. C-GSPN makes the operator practical through three improvements: (1) a fast GSPN CUDA kernel that fuses per-step launches into a single warp-specialized implementation with shared-memory tiling, coalesced access, and a compact multi-channel propagation, reaching over 90% of peak memory bandwidth and running up to 40--52x faster than the original GSPN implementation; (2) a compressed latent-space propagation block with fused normalization, which turns kernel-level speed into block- and model-level efficiency; and (3) a two-stage cross-operator distillation recipe that trains the new architecture from an attention teacher without the cost of from-scratch foundation-scale training. Distilled with 600M image-text pairs, C-GSPN matches an isomorphic ViT baseline with 15% fewer parameters, improves ADE20K segmentation by +2.1%, transfers to high resolution with a fraction of the data needed from scratch, and delivers a 4x end-to-end block speedup at 2K with single-pass, tiling-free inference.

==> sections/fig2_kernel.tex <==
% ============================================================================
%  Figure 2: GSPN kernel (baseline) vs. fast GSPN kernel (ours)
%  (a) GSPN kernel: per-column separate launches, HBM round-trips, no reuse
%  (b) fast GSPN kernel: single fused kernel, on-chip reuse of h_{i-1}, G_i
%  Rendered with TikZ (vector, on-brand). Included by sections/4__gspn2_kernel.tex
% ============================================================================
\definecolor{nvgreen}{HTML}{76B900}
\definecolor{nvgreenD}{HTML}{4E7A00}
\definecolor{hbmtan}{HTML}{C9BC8E}
\definecolor{featgrn}{HTML}{9FCB54}
\definecolor{cacheteal}{HTML}{1FA89B}
\definecolor{smemvio}{HTML}{9B6BC9}
\definecolor{regblue}{HTML}{6FA8DC}
\definecolor{warnred}{HTML}{C0392B}

\begin{tikzpicture}[
    font=\sffamily,
    >={Stealth[length=2.6mm]},
    reg/.style   ={draw=regblue!85!black, fill=regblue!28, rounded corners=1.5pt, line width=0.6pt},
    hbm/.style   ={draw=olive!60!black, fill=hbmtan!75, rounded corners=2pt, line width=0.7pt},
    feat/.style  ={draw=featgrn!60!black, fill=featgrn!55, rounded corners=1.5pt, line width=0.6pt},
    cache/.style ={draw=cacheteal!70!black, fill=cacheteal!30, rounded corners=2pt, line width=0.7pt},
    smem/.style  ={draw=smemvio!60!black, fill=smemvio!28, rounded corners=2pt, line width=0.7pt},
    ours/.style  ={draw=nvgreenD, fill=nvgreen!16, rounded corners=3pt, line width=1.1pt},
    lbl/.style   ={font=\sffamily\small},
    slbl/.style  ={font=\sffamily\footnotesize},
    ttl/.style   ={font=\sffamily\large\bfseries},
    flow/.style  ={->, line width=0.9pt, gray!55!black},
    redflow/.style={->, line width=1.2pt, warnred},
    grnflow/.style={->, line width=1.2pt, nvgreenD},
    panelbg/.style={draw=gray!35, fill=gray!4, rounded corners=5pt, line width=0.7pt},
]

\def\pb{10.3}  % x-origin of right panel

% =================================================================
% ============== PANEL (a): GSPN kernel (baseline) ================
% =================================================================
\begin{scope}
  \node[panelbg, minimum width=9.4cm, minimum height=8.2cm] (bgA) at (4.55,3.7) {};
  \node[ttl] at (4.55,7.55) {(a) GSPN kernel \;\normalfont\itshape(baseline)};

  % --- separate kernel launches (1D blocks) ---
  \node[reg, minimum width=1.7cm, minimum height=0.8cm] (kA1) at (1.8,6.35) {$K_{i\text{-}1}$};
  \node[reg, minimum width=1.7cm, minimum height=0.8cm] (kA2) at (3.85,6.35) {$K_{i}$};
  \node[reg, minimum width=1.7cm, minimum height=0.8cm] (kA3) at (5.9,6.35) {$K_{i\text{+}1}$};
  \node[lbl] at (7.3,6.35) {$\cdots$};
  \draw[decorate, decoration={brace, amplitude=5pt}, gray!55!black]
        (0.9,6.9) -- (7.7,6.9)
        node[midway, above=4pt, slbl, text=warnred]{a \emph{separate} kernel launch per column};

  % --- HBM ---
  \node[hbm, minimum width=3.6cm, minimum height=1.45cm, align=center] (hbmA) at (3.85,2.45)
        {\textbf{HBM (global memory)}\\[2pt] $X,\,G,\,H,\,B,\,\Lambda$};

  % round-trip arrows for the middle kernel
  \draw[redflow] ([xshift=-0.45cm]kA2.south) -- ([xshift=-0.45cm]hbmA.north)
        node[midway, left, slbl, text=warnred, align=right]{load\\$x_i,h_{i\text{-}1}$};
  \draw[redflow] ([xshift=0.55cm]hbmA.north) -- ([xshift=0.55cm]kA2.south)
        node[midway, right, slbl, text=warnred]{store $h_i$};

  % redundant traffic callout
  \node[slbl, text=warnred, align=center, fill=warnred!8, rounded corners=2.5pt,
        inner sep=3pt] at (7.0,3.9)
        {every step\\ round-trips\\ through HBM\\[1pt] \textbf{no on-chip}\\ \textbf{reuse}};

  % recurrence
  \node[lbl] at (4.0,0.62) {$h_i^{c}=\omega_i^{c}\,h_{i\text{-}1}^{c}+\lambda_i^{c}\odot x_i^{c}$};
\end{scope}

% =================================================================
% ============= PANEL (b): fast GSPN kernel (ours) ================
% =================================================================
\begin{scope}[shift={(\pb,0)}]
  \node[panelbg, minimum width=9.4cm, minimum height=8.2cm] (bgB) at (4.55,3.7) {};
  \node[ttl, text=nvgreenD] at (4.55,7.55) {(b) fast GSPN kernel \;\normalfont\itshape(ours)};

  % --- one fused kernel with inner loop over columns ---
  \node[ours, minimum width=7.8cm, minimum height=1.9cm] (fuse) at (4.3,6.0) {};
  \node[slbl, text=nvgreenD, anchor=north west] at ([xshift=3pt,yshift=-3pt]fuse.north west)
        {\textbf{single kernel:} one launch, inner loop over columns $i$};
  \node[feat, minimum width=1.35cm, minimum height=0.72cm] (s1) at (1.85,5.6) {\footnotesize step $i\text{-}1$};
  \node[feat, minimum width=1.35cm, minimum height=0.72cm] (s2) at (3.65,5.6) {\footnotesize step $i$};
  \node[feat, minimum width=1.35cm, minimum height=0.72cm] (s3) at (5.45,5.6) {\footnotesize step $i\text{+}1$};
  \node[lbl] at (6.75,5.6) {$\cdots$};
  \draw[grnflow] (s1) -- (s2);  \draw[grnflow] (s2) -- (s3);

  % --- on-chip region ---
  \node[draw=nvgreenD, dashed, rounded corners=4pt, line width=0.8pt,
        minimum width=5.6cm, minimum height=1.5cm] (chip) at (3.55,3.45) {};
  \node[slbl, text=nvgreenD, anchor=south west] at ([xshift=3pt,yshift=2pt]chip.north west)
        {\textbf{on-chip} (no HBM round-trip)};
  \node[smem, minimum width=2.3cm, minimum height=0.95cm, align=center] (sm) at (2.45,3.4)
        {\footnotesize shared memory\\[1pt] $h_{i\text{-}1}$ \;(reuse)};
  \node[cache, minimum width=2.1cm, minimum height=0.95cm, align=center] (rg) at (4.95,3.4)
        {\footnotesize registers\\[1pt] $G_i$ \;(reuse)};
  \draw[grnflow] (s2.south) -- ++(0,-0.55) -| (chip.north);

  % --- HBM (minimal traffic) ---
  \node[hbm, minimum width=2.9cm, minimum height=0.95cm, align=center] (hbmB) at (3.0,1.35)
        {\textbf{HBM}\;\; $X,\Lambda$};
  \draw[grnflow] ([xshift=0.55cm]hbmB.north) -- ([xshift=0.55cm]chip.south)
        node[midway, right, slbl, text=nvgreenD]{load $x$ once};
  \draw[grnflow] ([xshift=-0.6cm]chip.south) -- ([xshift=-0.6cm]hbmB.north)
        node[midway, left, slbl, text=nvgreenD, align=right]{store $h$\\once};

  % --- compact CUDA-layout note ---
  \node[draw=gray!45, fill=white, rounded corners=3pt, line width=0.6pt,
        align=center, slbl, text=gray!25!black] at (7.35,1.55)
        {\textbf{CUDA layout}\\ 2D $(\text{chunk},b,c)$ blocks\\ coalesced $\cdot$ 4 streams};
\end{scope}

% =================================================================
% ========================= shared legend =========================
% =================================================================
\begin{scope}[shift={(0.4,-0.85)}]
  \def\ly{0}
  \node[reg, minimum width=0.5cm, minimum height=0.34cm] (l1) at (0,\ly) {};
  \node[lbl, anchor=west] at (0.32,\ly) {ALU / register};
  \node[hbm, minimum width=0.5cm, minimum height=0.34cm] (l2) at (3.2,\ly) {};
  \node[lbl, anchor=west] at (3.52,\ly) {HBM};
  \node[feat, minimum width=0.5cm, minimum height=0.34cm] (l3) at (5.1,\ly) {};
  \node[lbl, anchor=west] at (5.42,\ly) {image / feature};
  \node[cache, minimum width=0.5cm, minimum height=0.34cm] (l4) at (8.5,\ly) {};
  \node[lbl, anchor=west] at (8.82,\ly) {L1/L2 cache};
  \node[smem, minimum width=0.5cm, minimum height=0.34cm] (l5) at (11.6,\ly) {};
  \node[lbl, anchor=west] at (11.92,\ly) {shared memory};
  \node[ours, minimum width=0.5cm, minimum height=0.34cm] (l6) at (15.0,\ly) {};
  \node[lbl, anchor=west] at (15.32,\ly) {fast GSPN (ours)};
  % 1D block icon
  \begin{scope}[shift={(18.6,\ly)}]
    \foreach \i in {0,1,2}{\node[reg, minimum width=0.28cm, minimum height=0.28cm, inner sep=0] at (\i*0.31,0) {};}
  \end{scope}
  \node[lbl, anchor=west] at (19.55,\ly) {1D block};
\end{scope}

\end{tikzpicture}

